Solving influence diagrams via efficient mixed-integer programming formulations and heuristics

In this paper, we propose novel mixed-integer linear programming (MIP) formulations to model decision problems posed as influence diagrams. We also present a novel heuristic that can be employed to warm start the MIP solver, as well as provide heuristic solutions to more computationally challenging problems. We provide computational results showcasing the superior performance of these improved formulations as well as the performance of the proposed heuristic. Lastly, we describe a novel case study showcasing decision programming as an alternative framework for modelling multi-stage stochastic dynamic programming problems.

==> sections/5-interface.tex <==
\section{Julia interface} 
\label{sec:interface}

The ideas and formulations presented in this paper have been implemented as a Julia \citep{Julia-2017} package. The main purpose of the package is to provide an interface through which a user can build an influence diagram and automatically convert it to a MILP model that can be solved using an off-the-shelf solver. This brings us to the main reasons for choosing Julia as the language of the package. Thanks to JuMP \citep{DunningHuchetteLubin2017} and MathOptInterface \citep{legat2022mathoptinterface}, implementing optimization problems in a general form is straightforward, and the models constructed in this way can be passed to many different solvers.

In order to create a user-friendly package that precludes a deeper understanding of MILP modeling by the user, we implemented a structure for influence diagrams and an interface for constructing them, demonstrated in Figure \ref{fig:code-nodes}. In that, we illustrate the implementation of the pig farm problem, originally proposed in \citet{lauritzen2001representing}. The influence diagram of the pig farm problem is presented in Figure \ref{fig:pigfarm}.
%
\begin{figure}
    \centering
    \include{figures/pigfarm}
    \caption{The influence diagram of the pig farm problem.}
    \label{fig:pigfarm}
\end{figure}

The influence diagram structure consists of nodes and their state spaces and information sets, as well as the corresponding probabilities and utility values. The interface includes functions for adding these elements into the influence diagram and type structures that guide the user to include the required information. For example, all node types require the user to define an information set for the node, even if it is empty (in the case of a root node). In turn, the function for adding nodes stops the user from accidentally including a node in its own information set, ensures that the names of all nodes are unique, and warns about redundant nodes. 

\begin{figure}[!ht]
    \centering
    \begin{lstlisting}[language = Julia]
    using JuMP, Gurobi, DecisionProgramming
    
    const N = 4
    
    diagram = InfluenceDiagram()
    
    # Syntax: 
    # ChanceNode(<name>, <information set>, <states>)
    # DecisionNode(<name>, <information set>, <states>)
    # ValueNode(<name>, <information set>)
    
    add_node!(diagram, ChanceNode("H1", [], ["ill", "healthy"]))
    for i in 1:N-1
        # Testing result
        add_node!(diagram, ChanceNode("T$i", ["H$i"], ["positive", "negative"]))
        # Decision to treat
        add_node!(diagram, DecisionNode("D$i", ["T$i"], ["treat", "pass"]))
        # Cost of treatment
        add_node!(diagram, ValueNode("C$i", ["D$i"]))
        # Health of next period
        add_node!(diagram, ChanceNode("H$(i+1)", ["H$(i)", "D$(i)"], ["ill", "healthy"]))
    end
    add_node!(diagram, ValueNode("MP", ["H$N"]))
    
    generate_arcs!(diagram)
    \end{lstlisting}
    \caption{Code to generate the nodes in the pig farm problem \citep{lauritzen2001representing}}
    \label{fig:code-nodes}
\end{figure}

Furthermore, specialised structures and functions (Figure \ref{fig:code-diagram}) for defining and adding chance nodes' conditional probabilities and value nodes' utility values ensure that these matrices have correct dimensions, that the probabilities sum to one and that utility values are defined for all information states of value nodes. The interface also includes a function for generating the arcs in the diagram and giving the nodes a topological order based on the information sets that the user has defined for them. This function also throws an error if the diagram has a directed cycle. 

\begin{figure}[!ht]
    \centering
    \begin{lstlisting}[language = Julia]
    # Add probabilities for node H1
    add_probabilities!(diagram, "H1", [0.1, 0.9])
    
    # Declare probability matrix for health nodes H_2, ... H_N
    X_H = ProbabilityMatrix(diagram, "H2")
    X_H["healthy", "pass", :] = [0.2, 0.8]
    X_H["healthy", "treat", :] = [0.1, 0.9]
    X_H["ill", "pass", :] = [0.9, 0.1]
    X_H["ill", "treat", :] = [0.5, 0.5]
    
    # Declare probability matrix for test result nodes T_1...T_{N-1}
    X_T = ProbabilityMatrix(diagram, "T1")
    X_T["ill", "positive"] = 0.8
    X_T["ill", "negative"] = 0.2
    X_T["healthy", "negative"] = 0.9
    X_T["healthy", "positive"] = 0.1
    
    for i in 1:N-1
        add_probabilities!(diagram, "T$i", X_T)
        add_probabilities!(diagram, "H$(i+1)", X_H)
    end
    
    for i in 1:N-1
        add_utilities!(diagram, "C$i", [-100.0, 0.0])
    end
    
    add_utilities!(diagram, "MP", [300.0, 1000.0])
    
    generate_diagram!(diagram)
    \end{lstlisting}
    \caption{Code to parametrize and generate an influence diagram}
    \label{fig:code-diagram}
\end{figure}

After the user has successfully generated an influence diagram, they can generate the model directly from the diagram structure, as shown in Figure \ref{fig:code-model}. The model is generated using specialised functions for declaring decision variables and constraints which merely require the (empty) JuMP model and the influence diagram structure as parameters. These functions include optional keyword arguments which allow the user to define forbidden and fixed subpaths, probability cuts and probability scaling for better computational performance. A significant advantage of implementing the framework using JuMP is that more advanced users can easily extend these models by adding new variables or constraints as needed. All of the features presented in this paper are implemented in the framework. These include valid inequalities as lazy constraints, a conditional Value-at-Risk objective function and the single policy update heuristic. 

\begin{figure}[!ht]
    \centering
    \begin{lstlisting}[language = Julia]
    model = Model(Gurobi.Optimizer)
    z = DecisionVariables(model, diagram)
    x_s = PathCompatibilityVariables(model, diagram, z)
    EV = expected_value(model, diagram, x_s)
    @objective(model, Max, EV)
    optimize!(model)
    \end{lstlisting}
    \caption{Code to solve the pig farm problem}
    \label{fig:code-model}
\end{figure}

Finally, the results of the optimization model can be extracted using a variety of functions. Figure \ref{fig:code-results} showcases arguably the most important of these, namely the functions for showing the optimal strategy. Other functions for analyzing results allow printing the distribution and statistics for the path utilities, and printing so-called state probabilities, that is, probabilities of given states occurring with the chosen strategy. For instance, in the pig farm problem, with the optimal strategy, the probability of the pig being healthy in stages 2, 3 and 4 is 73\%, 70.5\% and 69.5\%, respectively. 

\begin{figure}[!ht]
    \centering
    \begin{lstlisting}[language = Julia]
    Z = DecisionStrategy(z)
    S_probabilities = StateProbabilities(diagram, Z)
    
    print_decision_strategy(diagram, Z, S_probabilities)
    # Output:
    # ┌────────────────┬────────────────┐
    # │ State(s) of T1 │ Decision in D1 │
    # ├────────────────┼────────────────┤
    # │ positive       │ pass           │
    # │ negative       │ pass           │
    # └────────────────┴────────────────┘
    # ┌────────────────┬────────────────┐
    # │ State(s) of T2 │ Decision in D2 │
    # ├────────────────┼────────────────┤
    # │ positive       │ treat          │
    # │ negative       │ pass           │
    # └────────────────┴────────────────┘
    # ┌────────────────┬────────────────┐
    # │ State(s) of T3 │ Decision in D3 │
    # ├────────────────┼────────────────┤
    # │ positive       │ treat          │
    # │ negative       │ pass           │
    # └────────────────┴────────────────┘
    \end{lstlisting}
    \caption{Code to obtain the optimal strategy for the pig farm problem}
    \label{fig:code-results}
\end{figure}
